RuleReasoner: Reinforced Rule-based Reasoning via Domain-aware Dynamic Sampling

Rule-based reasoning is acknowledged as one of the fundamental problems of reasoning. While recent studies show that large reasoning models (LRMs) have remarkable reasoning capabilities enhanced by reinforcement learning (RL), real applications still face severe challenges due to variations in rule formats, types, and complexity. To mitigate this issue, we introduce RuleReasoner, an effective method for rule-based reasoning via a wide collection of curated tasks and a novel domain-aware dynamic sampling approach in RL. Specifically, RuleReasoner resamples each training batch by updating the domain weights based on historical rewards. This facilitates domain balance and active learning schedules for RL, obviating static mix-training engineered by human. Evaluations on in-distribution (ID) and out-of-distribution (OOD) benchmarks reveal that RuleReasoner outperforms frontier LRMs by a significant margin ($\Delta$4.1% on eight ID tasks and $\Delta$10.4% on three OOD tasks over OpenAI-o1). Notably, our approach also exhibits higher computational efficiency compared to prior methods.

==> figure/main_results.tex <==
\begin{figure*}[t]
  \centering
  \resizebox{1.0\linewidth}{!}{\includegraphics{figure/raw/main_results.pdf}}
  \caption{\ourmethod versus leading open-weights and proprietary large reasoning models on eight rule-based logical reasoning benchmarks. \yang{replot with a larger multi-column table}}
  \label{fig:main-results}
\end{figure*}

==> figure/training_datasize_impact.tex <==
% \begin{figure}[t]
%   \centering
%   \resizebox{1\linewidth}{!}{\includegraphics{figure/raw/training_datasize_impact.pdf}}
%   \caption{Comparison of the impact on scaling training data size.}
%   \label{fig:training_datasize_impact}
% \end{figure}

==> table/ablation_rules.tex <==
\begin{table}[htbp]
  \centering
  \begin{tabular}{lcc}
    \toprule 
    {Model} & $\text{Test}_\text{w/ rule}$ & $\text{Test}_\text{w/o rule}$ \\
    \midrule 
    $\text{Train}_\text{w/ rule}$ & * & *  \\
    $\text{Train}_\text{w/o rule}$ & * & *  \\
    \bottomrule
  \end{tabular}
  \caption{Ablation results on the impact of rules. [TODO] replace this table with a confusion matrix.}
  \label{tab:ablation_rules}
\end{table}

==> table/difficulty_aware_performance.tex <==
\begin{table}[htbp]
  \centering
  \begin{tabular}{lccc}
    \toprule 
    {OOD Test} & {Easy} & {Medium} & {Hard} \\
    \midrule 
    ProverQA & * & *  & * \\
    BBH & * & *  & * \\
    BBEH & * & *  & * \\
    \bottomrule
  \end{tabular}
  \caption{Performance across varying difficulty.}
  \label{tab:difficulty_performance}
\end{table}

==> table/in_domain_results.tex <==
\begin{table*}[htbp]
  \centering
  \small
  \label{tab:id_performance}
  \begin{tabular}{l cccc cc}
    \toprule
    \textbf{In-domain} &  
    \textbf{ProntoQA} & \textbf{ProofWriter} & \textbf{FOLIO} &
    %\textbf{Clutrr} &
    %\textbf{Boxes} &
    %\textbf{AR-LSAT} &
    \textbf{LogicNLI} &
    \textbf{LogicalDeduction} & \textbf{Avg. $\Delta^\dagger$} \\
    \midrule
    OpenAI-o1 & & & & & & \\
    OpenAI-o3-mini & & & & & & \\
    Gemini-2.5-Pro & & & & & & \\
    Claude-3.7-Sonnet & & & & & & \\
    % \midrule
    DeepSeek-R1 & & & & & & \\
    % QwQ-32B & & & & & & \\
    % DeepSeek-Qwen-32B & & & & & & \\
    \midrule
    \ourmodel & \rbox{44.6} \tiny{-31.0} & \rbox{\textbf{92.0}} \tiny{+12.4} & \gbox{\textbf{71.6}} \tiny{+14.8} & \rbox{50.0} \tiny{-13.6} & \rbox{-2.0}\tiny{+6.4} \\
    + Rules & \rbox{31.0} \tiny{-2.6} & \rbox{63.4} \tiny{-16.2} & \rbox{42.8} \tiny{-14.0} & \gbox{\textbf{70.0}} \tiny{+6.4} & \rbox{-11.4}\tiny{+6.4} \\
    + Dynamic Sampling & \gbox{\textbf{97.0}} \tiny{+21.4} & \gbox{\textbf{90.6}} \tiny{+44.0} & \gbox{\textbf{68.2}} \tiny{+34.6} & \rbox{68.5} \tiny{+5.0} & \gbox{\textbf{+7.5}}\tiny{+6.4} \\
    \hdashline
    \ourmodellarge & \rbox{44.6} \tiny{-31.0} & \rbox{\textbf{92.0}} \tiny{+12.4} & \gbox{\textbf{71.6}} \tiny{+14.8} & \rbox{50.0} \tiny{-13.6} & \rbox{-2.0}\tiny{+6.4} \\
    + Rules & \rbox{31.0} \tiny{-2.6} & \rbox{63.4} \tiny{-16.2} & \rbox{42.8} \tiny{-14.0} & \gbox{\textbf{70.0}} \tiny{+6.4} & \rbox{-11.4}\tiny{+6.4} \\
    + Dynamic Sampling & \gbox{\textbf{97.0}} \tiny{+21.4} & \gbox{\textbf{90.6}} \tiny{+44.0} & \gbox{\textbf{68.2}} \tiny{+34.6} & \rbox{68.5} \tiny{+5.0} & \gbox{\textbf{+7.5}}\tiny{+6.4} \\
    \bottomrule
  \end{tabular}
  \caption{In-domain reasoning performance comparison}
  %\vspace{0.5em}
\end{table*}

==> table/sampling_method_comparison.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{llcccccc}
\toprule
\textbf{Task} & \textbf{Thinking} & \textbf{BF (tokens)} & \textbf{Pass@K} & \multicolumn{3}{c}{\textbf{Selection Methods (Pass@1)}} \\
\cmidrule(lr){5-7}
& & & & \textbf{Majority Voting} & \textbf{Confidence + Voting} \\
\midrule
\multirow{2}{*}{AIME 2024} & \textit{Thinking} &  &  &  & \textbf{} \\
& \textit{NoThinking} &  &  &  & \textbf{} \\
\midrule
\multirow{2}{*}{AIME 2025} & \textit{Thinking} &  &  & \textbf{} &  \\
& \textit{NoThinking} &  &  & \textbf{} &  \\
\midrule
\multirow{2}{*}{AMC 2023} & \textit{Thinking} &  &  &  \\
& \textit{NoThinking} &  &  & \textbf{} \\
\bottomrule
\end{tabular}
\caption{Performance across different tasks, thinking modes, and selection methods.}
\label{tab:sampling_method_comparison}
\end{table*}
